Racial Disparities in Debt Collection

This paper shows that black and Hispanic borrowers are 39% more likely to experience a debt collection judgment than white borrowers, even after controlling for credit scores and other relevant credit attributes. The racial gap in judgments is more pronounced in areas with a high density of payday lenders, a high share of income-less households, and low levels of tertiary education. State-level measures of racial discrimination cannot explain the judgment gap, nor can neighborhood-level differences in the previous share of contested judgments or cases with attorney representation. A back-of-the-envelope calculation suggests that closing the racial wealth gap could significantly reduce the racial disparity in debt collection judgments.

==> Tables/Tables_neighborhood/results_debt_portfolio_individual.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios (Individual Data)\label{tab:individual_portfolio_prob}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Probability of Being Black      &      0.0072\sym{***}&      0.0073\sym{***}&      0.0082\sym{***}&      0.0047\sym{***}&      0.0040\sym{***}\\
                    &    (0.0006)         &    (0.0006)         &    (0.0006)         &    (0.0006)         &    (0.0006)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\ \hline 
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12939752      &12939752      &12939752      &12939752      &12939752      \\
$R^2$               &      0.0638         &      0.0631         &      0.0614         &      0.0711         &      0.0727         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment. County and quarter fixed effects are included in all specifications. Observations from the Experian sample, data available from 2013 until 2018Q2. We use the individuals age and ZIP code to infer their probability of being black.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> Tables/Tables_neighborhood/results_debt_portfolio_individual_zip.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios (Individual Data): ZIP\label{tab:individual_portfolio_zip}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP     &      0.0065\sym{***}&      0.0066\sym{***}&      0.0072\sym{***}&      0.0054\sym{***}&      0.0048\sym{***}\\
                    &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         \\
\hline
Observations        &12935791       &12935791       &12935791       &12935791       &12935791       \\
$R^2$               &      0.0638         &      0.0632         &      0.0615         &      0.0711         &      0.0728         \\ \hline \hline
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\ \hline 
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]

\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment. County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. 
\end{tablenotes}
\end{threeparttable}
\end{table}



==> Tables/Tables_neighborhood/results_judgments_individual.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (Individual Judgment Data) \label{tab:individual}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Probability of Being Black    &      0.0479\sym{***}&      0.0469\sym{***}&      0.0088\sym{***}&      0.0084\sym{***}\\
                    &    (0.0018)         &    (0.0018)         &    (0.0018)         &    (0.0018)         \\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Income &                            &     X &                     &    X\\
Credit Score                     &                     &                     &     X&     X\\
\hline & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12939752        &12939752        &12939752        &12939752        \\
$R^2$               &      0.0303         &      0.0307         &      0.0611         &      0.0612         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment.  County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. We use the individuals age and ZIP code to infer their probability of being black.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_neighborhood/results_judgments_individual_zip.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (Individual Data): ZIP \label{tab:individual_zip}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP    &      0.0262\sym{***}&      0.0258\sym{***}&      0.0075\sym{***}&      0.0073\sym{***}\\
                    &    (0.0014)         &    (0.0014)         &    (0.0014)         &    (0.0014)         \\ \hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Income &                            &     X &                     &    X\\
Credit Score                     &                     &                     &     X&     X\\
\hline & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12935791    &12935791    &12935791    &12935791    \\
$R^2$               &      0.0294         &      0.0298         &      0.0611         &      0.0612         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment.  County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_neighborhood/results_judgments_neighborhood_bisg.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Creditworthiness\label{tab:creditworthiness_bisg}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: BISG&      1.2637\sym{***}&      0.7413\sym{***}&      0.9180\sym{***}&      0.6791\sym{***}&      0.6283\sym{***}&      0.6899\sym{***}\\
                    &    (0.1571)         &    (0.1505)         &    (0.1290)         &    (0.1401)         &    (0.1347)         &    (0.0310)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income Details      &                     &           X         &                     &           X         &           X         &                     \\
Credit Quintiles    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\ 
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0001         &       .0005         &           0         \\
Observations        &   7361        &   7361        &   7015       &   7015        &   7015        &   6103       \\
$R^2$               &      0.5799         &      0.6585         &      0.6207         &      0.6661         &      0.6860         &      0.6739         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_neighborhood/results_judgments_neighborhood_other_areas.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (NJ and IL Data) \label{tab:creditworthiness_nj_il}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                       &\multicolumn{6}{c}{Judgment Rate}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP  &      0.9667\sym{***}&      0.8630\sym{***}&      0.3650\sym{***}&      0.5833\sym{***}&      0.2981\sym{***}&      0.3978\sym{***}\\
                    &    (0.1297)         &    (0.1058)         &    (0.0940)         &    (0.0876)         &    (0.0885)         &    (0.0844)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income      &                     &           X         &                     &           X         &           X         &                     \\
Credit Score   &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &           0         &       .0008         &           0         \\
Observations        &   3397        &   3397        &   3103        &   3103        &   3103        &   2118        \\
$R^2$               &      0.8733         &      0.8994         &      0.8909         &      0.9034         &      0.9089         &      0.9119         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 30.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_neighborhood/summary_tab1_individual.tex <==
\begin{table}[th]\centering
  \begin{threeparttable}
 \small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics for Individual Level Experian Data\label{tab:summary_statistics_individual}}
\begin{tabular}{l*{3}{cc}}
\hline\hline
                    &\multicolumn{1}{c}{Black}&\multicolumn{1}{c}{Non-Black}&\multicolumn{1}{c}{Difference}\\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textcolor{white}{...}Share with Judgments           &        0.06&        0.03&       -0.03\sym{***}\\
                    &      (0.23)&      (0.16)&                     \\
 \textcolor{white}{...}Household Income   &       43.82&       51.61&        7.79\sym{***}\\
                    &     (71.09)&     (52.32)&                     \\
 \textcolor{white}{...}Credit Score      &      610.87&      684.70&       73.83\sym{***}\\
                    &    (120.38)&    (113.25)&                     \\
 \textcolor{white}{...}90+ DPD Debt Balances    &     3933.21&     2109.77&    -1823.44\sym{***}\\
                    &  (31475.04)&  (23339.70)&                     \\
 \textcolor{white}{...}Age &       47.92&       49.01&        1.09\sym{***}\\
                    &     (16.34)&     (16.54)&                     \\
    \hline
Observations     &      707919&    12229556&    12937475         \\
\hline\hline
\end{tabular}

   \begin{tablenotes}
     \small
    \item Notes:  Individual level common support sample. Standard deviations are in parenthesis. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)
   \end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_noncommon/results_alternative_credit_risk_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Credit Score: Entire Sample\label{tab:pp_off_common}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.7143\sym{***}&      1.2269\sym{***}&      0.9769\sym{***}&      0.8158\sym{***}&      1.0181\sym{***}\\
                    &    (0.2216)         &    (0.1776)         &    (0.1921)         &    (0.1734)         &    (0.0332)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &           X         &                     \\
Income              &                     &                     &           X         &           X         &                     \\
Default Probability &                     &           X         &           X         &           X         &           X         \\
Lagged Baseline Controls&                     &                     &                     &                     &           X         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &       .0005         &           0         \\
Observations        &   6666       &   6666       &   6352       &   6017       &   5275       \\
$R^2$               &      0.5779         &      0.6325         &      0.6991         &      0.7230         &      0.7388         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications. Column (5) controls for lagged default probability instead of default probability.  Default probability data is available from 2006.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_noncommon/results_alternative_dependent_neighborhood_off_common_support.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Alternative Dependent Variables: Entire Sample\label{tab:judgment_alternative_off_common}}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
&\multicolumn{1}{c}{Judgments/Cases}&\multicolumn{2}{c}{Judgment: Low Income}&\multicolumn{2}{c}{Judgment: Low Credit }&\multicolumn{2}{c}{Judgment: Winsorized} \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &       0.026\sym{**}&       2.830\sym{***}&       2.607\sym{***}&       0.506\sym{***}&       0.499\sym{***} &       0.707\sym{***}&       0.693\sym{***}\\
                  &     (0.010)           &     (0.680)         &     (0.615)         &     (0.117)         &     (0.121)      &     (0.160)         &     (0.150)            \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Population Weighted &                 &             X        &                    &             X        &                 &    X                 &                     \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Boostrap p-value &       .0146        &       .0004         &       .0002         &       .0016         &        .001             &       .0004         &       .0002     \\
Observations        &    7484        &    7484        &    7484        &    7484        &    7464        &    7464        &    7484        \\
$R^2$               &       0.185           &       0.671         &       0.551         &       0.754         &       0.576      &       0.702         &       0.519          \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects, attorney representation included in all specifications. For Column (1) our dependent variable is the fraction of cases that result in a judgment, for Columns (2-3), our outcome variable is judgments per 100 individuals with tax filings under \$25,000 USD, for Columns (4-5) our outcome variable is judgments per 100 individuals with subprime credit, and for Columns (6-7) we winsorize our main outcome variable, judgments per 100 individuals, at the 99th percentile.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/Tables_noncommon/results_credit_markets_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Access to Credit Markets: Entire Sample\label{tab:access_to_credit_off_common}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.0704\sym{***}&      1.0699\sym{***}&      1.0706\sym{***}&      0.9528\sym{***}&      0.9185\sym{***}\\
                    &    (0.1436)         &    (0.1434)         &    (0.1437)         &    (0.1256)         &    (0.1279)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Broadband           &                     &      0.0374\sym{*}  &                     &                     &                     \\
                    &                     &    (0.0214)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Unscored            &                     &                     &      0.1337         &                     &                     \\
                    &                     &                     &    (0.2643)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (5 miles)     &                     &                     &                     &     -0.0047\sym{***}&                     \\
                    &                     &                     &                     &    (0.0008)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (5 miles)&                     &                     &                     &      0.0161\sym{***}&                     \\
                    &                     &                     &                     &    (0.0026)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (10 miles)    &                     &                     &                     &                     &     -0.0021\sym{***}\\
                    &                     &                     &                     &                     &    (0.0003)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (10 miles)&                     &                     &                     &                     &      0.0083\sym{***}\\
                    &                     &                     &                     &                     &    (0.0009)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &           0         \\
\hline 
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &   4488       &   4488       &   4488       &   4488       &   4488       \\
$R^2$               &      0.8248         &      0.8250         &      0.8248         &      0.8335         &      0.8344         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_noncommon/results_housing_market_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Local Housing Markets: Entire Sample\label{tab:access_to_housing_off_common}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      0.9253\sym{***}&      0.8022\sym{***}&      0.7012\sym{***}&      0.6903\sym{***}\\
                    &    (0.1591)         &    (0.1401)         &    (0.1590)         &    (0.1563)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA: Share Rejected&                     &      1.2362\sym{***}&                     &                     \\
                    &                     &    (0.3948)         &                     &                     \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Zillow: Single Family House&                     &                     &                     &     -0.0040\sym{***}\\
                    &                     &                     &                     &    (0.0007)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA Available      &           X         &           X         &                     &                     \\
Zillow Available    &                     &                     &           X         &           X         \\ \hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &       .0003         &       .0002         &       .0001         \\
Observations        &   4171      &   4171      &   5679      &   5679      \\
$R^2$               &      0.7764         &      0.7806         &      0.6960         &      0.7018         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> Tables/Tables_noncommon/results_judgments_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores: Entire Sample \label{tab:creditworthiness_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.5127\sym{***}&      0.8940\sym{***}&      1.0934\sym{***}&      0.8200\sym{***}&      0.7071\sym{***}&      0.8402\sym{***}\\
                    &    (0.2148)         &    (0.1912)         &    (0.1741)         &    (0.1816)         &    (0.1612)         &    (0.0325)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income Details      &                     &           X         &                     &           X         &           X         &                     \\
Credit Quintiles    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0006         &       .0005         &           0         \\
Observations        &   9788     &   9020     &   7837     &   7527     &   7484     &   6737     \\
$R^2$               &      0.5805         &      0.6694         &      0.6304         &      0.6814         &      0.7016         &      0.6903         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_noncommon/results_other_races_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Other Demographic Groups: Entire Sample\label{tab:race_other_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      2.3723\sym{***}&      1.5447\sym{***}&      1.9561\sym{***}&      1.4328\sym{***}&      1.4930\sym{***}&      1.5590\sym{***}\\
                    &    (0.3076)         &    (0.3300)         &    (0.2724)         &    (0.3088)         &    (0.2859)         &    (0.0557)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Asian: ZIP    &     -5.1481\sym{***}&     -2.9361\sym{***}&     -4.4323\sym{***}&     -2.8328\sym{***}&     -0.9491\sym{*}  &     -3.0248\sym{***}\\
                    &    (0.9695)         &    (0.6906)         &    (1.0057)         &    (0.7438)         &    (0.5175)         &    (0.3856)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Hispanic: ZIP &      1.3980\sym{***}&     -0.3906\sym{***}&      0.8922\sym{***}&     -0.4970\sym{***}&      0.4932\sym{***}&     -0.4124\sym{**} \\
                    &    (0.1707)         &    (0.1407)         &    (0.1666)         &    (0.1541)         &    (0.1589)         &    (0.1670)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income    &                     &           X         &                     &           X         &           X         &                     \\
Credit Score    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p$_{\text{Black}}$&           0         &           0         &           0         &       .0006         &           0         &           0         \\
Wild Cluster Bootstrap p$_{\text{Hispanic}}$&           0         &       .0098         &       .0002         &       .0038         &       .0036         &       .0298         \\
Wild Cluster Bootstrap p$_{\text{Asian}}$&           0         &       .0001         &       .0013         &       .0018         &        .092         &           0         \\
Observations        &   9788       &   9020       &   7837       &   7527       &   7484       &   6737       \\
$R^2$               &      0.6472         &      0.6868         &      0.6692         &      0.6968         &      0.7138         &      0.7068         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/Tables_noncommon/results_plaintiff_type_neighborhood_off_common_support.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Plaintiff Type: Entire Sample\label{tab:plaintiff_type_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Debt Buyer}&\multicolumn{1}{c}{Major Bank}&\multicolumn{1}{c}{Medical}&\multicolumn{1}{c}{High-Cost }&\multicolumn{1}{c}{Misc.}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &       0.707\sym{***}&       0.220\sym{***}&       0.052\sym{*}  &       0.045         &       0.116\sym{***}&       0.322\sym{***}\\
                    &     (0.161)         &     (0.050)         &     (0.029)         &     (0.052)         &     (0.022)         &     (0.077)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Mean                &       1.325         &        .584         & 0.489         &        .304         &        .079         &        .152         \\
Effect Size         &53.4        &        37.6         &        10.7         &          15         &         146         &       211.3         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0005         &       .0003         &       .1048         &.5348         &           0         &       .0001         \\
Observations        &    7484        &    7484        &    7484        &    7484        &    7484        &    7484        \\
$R^2$               &       0.702         &       0.710         &       0.734         &       0.623         &       0.607         &       0.534         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/Tables_noncommon/results_race_proxies_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Proxy for Race: Entire Sample\label{tab:race_proxies_off_common}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.4731\sym{***}&                     &                     &                     \\
                    &    (0.2890)         &                     &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &                     &      0.7071\sym{***}&                     &                     \\
                    &                     &    (0.1612)         &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: BISG   &                     &                     &      1.3774\sym{***}&                     \\
                    &                     &                     &    (0.2604)         &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: BISG&                     &                     &                     &      0.6305\sym{***}\\
                    &                     &                     &                     &    (0.1284)         \\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &       .0005         &       .0001         &       .0002         \\
Observations        &   7484        &   7484        &   7479        &   7479        \\
$R^2$               &      0.7133         &      0.7016         &      0.7147         &      0.7027         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> Tables/Tables_share/results_alternative_credit_risk_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Credit Score: Share Black\label{tab:pp_share_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP &      1.6996\sym{***}&      0.8755\sym{***}&      0.9238\sym{***}&      0.7283\sym{***}&      0.8163\sym{***}\\
                    &    (0.2524)         &    (0.1223)         &    (0.1388)         &    (0.1754)         &    (0.0525)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &           X         &                     \\
Income              &                     &                     &           X         &           X         &                     \\
Default Probability &                     &           X         &           X         &           X         &           X         \\
Lagged Baseline Controls&                     &                     &                     &                     &           X         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0095         &       .0015         &       .0159         &           0         &           0         \\
Observations        &   2088        &   2088        &   2088        &   2088        &   1611        \\
$R^2$               &      0.6071         &      0.7032         &      0.7434         &      0.7623         &      0.8124         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications. Column (5) controls for lagged default probability instead of default probability.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_share/results_alternative_dependent_neighborhood_share_black.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Alternative Dependent Variables: Share Black\label{tab:judgment_alternative_share_black}}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
&\multicolumn{1}{c}{Judgments/Cases}&\multicolumn{2}{c}{Judgment: Low Income}&\multicolumn{2}{c}{Judgment: Low Credit }&\multicolumn{2}{c}{Judgment: Winsorized} \\
\hline
& & & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP &       0.072\sym{***}   &       6.160\sym{***}&       4.467\sym{***}&       1.002\sym{***}&       0.747\sym{***} &       1.476\sym{***}&       1.096\sym{***}\\
                 &     (0.015)               &     (1.226)         &     (0.815)         &     (0.210)         &     (0.175)  &     (0.283)         &     (0.204)             \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Population Weighted &                  &                  X         &                     &         X           &                    &     X  &                  \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Boostrap p-value&           0                 &           0         &       .0004         &       .0003         &           0     &           0         &           0     \\

Observations        &    7019      &    7019      &    7019         &    6999      &    6999      &    7019     &    7019    \\
$R^2$           &       0.174               &       0.671         &       0.551         &       0.752         &       0.576     &       0.697         &       0.514           \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Regressions are weighted by population only in Columns (2), (4), and (6). Observations on the entire Missouri sample. Baseline controls, county, year fixed effects, and attorney representation included in all specifications. For Column (1) our dependent variable is the fraction of cases that result in a judgment, for Columns (2-3), our outcome variable is judgments per 100 individuals with tax filings under \$25,000 USD, for Columns (4-5) our outcome variable is judgments per 100 individuals with subprime credit, and for Columns (6-7) we winsorize our main outcome variable, judgments per 100 individuals, at the 99th percentile.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/Tables_share/results_credit_markets_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Access to Credit Markets: Share Black \label{tab:access_to_credit_share_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      2.1184\sym{***}&      2.1157\sym{***}&      2.1185\sym{***}&      1.9213\sym{***}&      2.0197\sym{***}\\
                    &    (0.2550)         &    (0.2546)         &    (0.2551)         &    (0.2065)         &    (0.2115)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Broadband           &                     &      0.0531\sym{**} &                     &                     &                     \\
                    &                     &    (0.0223)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Unscored            &                     &                     &      0.0927         &                     &                     \\
                    &                     &                     &    (0.2716)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (5 miles)     &                     &                     &                     &     -0.0053\sym{***}&                     \\
                    &                     &                     &                     &    (0.0010)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (5 miles)&                     &                     &                     &      0.0116\sym{***}&                     \\
                    &                     &                     &                     &    (0.0028)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (10 miles)    &                     &                     &                     &                     &     -0.0019\sym{***}\\
                    &                     &                     &                     &                     &    (0.0003)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (10 miles)&                     &                     &                     &                     &      0.0028\sym{**} \\
                    &                     &                     &                     &                     &    (0.0014)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &           0         \\
\hline 
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &   4183       &   4183       &   4183       &   4183       &   4183       \\
$R^2$               &      0.8371         &      0.8375         &      0.8371         &      0.8447         &      0.8460         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_share/results_debt_portfolio_neighborhood_other_areas_share_black.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Debt Portfolios: Share Black (NJ and IL Data)\label{tab:debt\_composition\_share\_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                    &\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}\\
\hline
fraction\_black      &      0.6786\sym{***}&      0.6632\sym{***}&      0.7179\sym{***}&      0.6930\sym{***}&      0.6875\sym{***}\\
                    &    (0.1541)         &    (0.1522)         &    (0.1568)         &    (0.1596)         &    (0.1565)         \\
\hline
Wild Cluster Bootstrap p-value&           0         &       .0001         &       .0001         &           0         &       .0001         \\
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
Observations        &   3103         &   3103         &   3103         &   3103         &   3103         \\
$R^2$               &      0.9113         &      0.9121         &      0.9111         &      0.9118         &      0.9153         \\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize Observations on the common support sample; estimated by Gradient Boosted Treed with five-fold cross-validation. Since the effective number of clusters is small, Wild Cluster Bootstrap p-values are reported for our main parameter of interest. Baseline controls, county, and year fixed effects included in all specifications.}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> Tables/Tables_share/results_housing_market_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Local Housing Markets: Share Black\label{tab:access_to_housing_share_black}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.8918\sym{***}&      1.8166\sym{***}&      1.5111\sym{***}&      1.4096\sym{***}\\
                    &    (0.2836)         &    (0.2818)         &    (0.2957)         &    (0.3001)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA: Share Rejected&                     &      0.3642         &                     &                     \\
                    &                     &    (0.3448)         &                     &                     \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Zillow: Single Family House&                     &                     &                     &     -0.0046\sym{***}\\
                    &                     &                     &                     &    (0.0013)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA Available      &           X         &           X         &                     &                     \\
Zillow Available    &                     &                     &           X         &           X         \\ \hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &       .0001         \\
Observations        &   3846        &   3846        &   5231        &   5231        \\
$R^2$               &      0.7765         &      0.7768         &      0.6898         &      0.6953         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> Tables/Tables_share/results_judgments_neighborhood_fraction_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores: Share Black \label{tab:creditworthiness_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\
Share Black: ZIP    &      2.4081\sym{***}&      1.6669\sym{***}&      1.9877\sym{***}&      1.5634\sym{***}&      1.4731\sym{***}&      1.7233\sym{***}\\
                    &    (0.2939)         &    (0.3308)         &    (0.2640)         &    (0.3064)         &    (0.2865)         &    (0.0583)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income      &                     &           X         &                     &           X         &           X         &                     \\
Credit Score   &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0001         &       .0001         &           0         \\
Observations        &   7365        &   7365        &   7019        &   7019        &   7019        &   6105        \\
$R^2$               &      0.6403         &      0.6769         &      0.6559         &      0.6816         &      0.6965         &      0.6921         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_share/results_judgments_neighborhood_other_areas_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (NJ and IL Data): Share Black \label{tab:creditworthiness_nj_il_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP      &      1.4889\sym{***}&      1.3818\sym{***}&      0.6564\sym{***}&      1.0221\sym{***}&      0.6958\sym{***}&      0.7178\sym{***}\\
                    &    (0.2252)         &    (0.1722)         &    (0.1593)         &    (0.1408)         &    (0.1581)         &    (0.1508)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income    &                     &           X         &                     &           X         &           X         &                     \\
Credit Score    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &       .0001         &           0         \\
Observations        &   3397         &   3397         &   3103         &   3103         &   3103         &   2118         \\
$R^2$               &      0.8815         &      0.9031         &      0.8919         &      0.9051         &      0.9097         &      0.9125         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.6. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample; estimated by Gradient Boosted Treed with five-fold cross-validation. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/Tables_share/results_plaintiff_type_neighborhood_share_black.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Plaintiff Type: Share Black\label{tab:plaintiff_type_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Debt Buyer}&\multicolumn{1}{c}{Major Bank}&\multicolumn{1}{c}{Medical}&\multicolumn{1}{c}{High-Cost }&\multicolumn{1}{c}{Misc.}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &       1.473\sym{***}&       0.483\sym{***}&       0.104\sym{**} &       0.024         &       0.277\sym{***}&       0.645\sym{***}\\
                    &     (0.286)         &     (0.096)         &     (0.051)         &     (0.079)         &     (0.044)         &     (0.144)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &           0         &       .0604         &       .8287         &           0         &           0         \\
Observations        &    7019        &    7019        &    7019        &    7019        &    7019        &    7019        \\
$R^2$               &       0.697         &       0.706         &       0.726         &       0.612         &       0.625         &       0.547         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications. Effect size computed for going from 0\% share black to 100\%.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/tab_4.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and Judgments}\label{table:4}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{5}{c}{Judgment Outstanding}&\multicolumn{1}{c}{Judgment Petitioned}&\multicolumn{1}{c}{Judgment Satisfied}\\

\hline
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female           &      0.0080         &      0.0037         &      0.0086         &      0.0397         &     -0.0059         &      0.0036         &      0.0063         \\
                    &    (0.0111)         &    (0.0138)         &    (0.0136)         &    (0.0571)         &    (0.0067)         &    (0.0098)         &    (0.0061)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority         &      0.1237\sym{***}&      0.1156\sym{***}&      0.0496\sym{**} &      0.1373\sym{*}  &      0.0194         &      0.0220         &      0.0120         \\
                    &    (0.0202)         &    (0.0246)         &    (0.0238)         &    (0.0756)         &    (0.0122)         &    (0.0178)         &    (0.0103)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age                 &     -0.0017\sym{***}&     -0.0018\sym{***}&      0.0008\sym{*}  &      0.0025         &      0.0003         &     -0.0002         &     -0.0003         \\
                    &    (0.0003)         &    (0.0004)         &    (0.0004)         &    (0.0020)         &    (0.0002)         &    (0.0003)         &    (0.0002)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$  &                     &                     &     -0.0024\sym{***}&     -0.0044\sym{***}&     -0.0004\sym{***}&     -0.0013\sym{***}&     -0.0002\sym{***}\\
                    &                     &                     &    (0.0002)         &    (0.0005)         &    (0.0001)         &    (0.0001)         &    (0.0000)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$            &                     &                     &      0.0019\sym{***}&      0.0011         &      0.0019         &      0.0011\sym{**} &     -0.0002         \\
                    &                     &                     &    (0.0006)         &    (0.0008)         &    (0.0020)         &    (0.0004)         &    (0.0002)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$           &                     &                     &     -0.0002\sym{***}&     -0.0006\sym{***}&     -0.0000         &     -0.0001\sym{***}&     -0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0002)         &    (0.0000)         &    (0.0000)         &    (0.0000)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Judgment Outstanding$_{t-1}$      &                     &                     &      0.0216         &     -0.8370\sym{***}&     -0.2061         &     -0.0466         &      0.6217\sym{***}\\
                    &                     &                     &    (0.0991)         &    (0.1410)         &    (0.1615)         &    (0.0639)         &    (0.0775)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.1956\sym{***}&      0.2067\sym{***}&      1.8568\sym{***}&      3.0859\sym{***}&      0.3312\sym{***}&      0.9873\sym{***}&      0.1673\sym{***}\\
                    &    (0.0171)         &    (0.0219)         &    (0.1186)         &    (0.3127)         &    (0.0621)         &    (0.0794)         &    (0.0353)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469015       & 468754       & 468753       & 122640       & 345323       & 468753       & 468753       \\
Mean of DV (Minority=0)           &      0.1258         &      0.1258         &      0.1258         &      0.4817         &      0.0187         &      0.0615         &      0.0249         \\
$R^2$               &      0.0044         &      0.0362         &      0.0385         &      0.0744         &      0.0339         &      0.0356         &      0.0379         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\item This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment outstanding (column 1-5), petitioned (column 6) or satisfied (column 7). The sample is quarterly credit report data. Columns 4 and 5 focus specifically on applicants with subprime and prime credit scores, respectively. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/tab_6.tex <==
\begin{sidewaystable}[!h]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and Judgments using ZCTA5 Demographics}\label{table:4}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{3}{c}{Judgment Outstanding} \\ 
                    & \underline{Full Sample} & \underline{Mortgagor} & \underline{Non-Mortgagor}\\

\hline
& & & \\[\dimexpr-\normalbaselineskip+3pt]
ZIP Minority Share        &      0.1646\sym{***}&      0.1821\sym{***}&      0.1470\sym{***}\\
                    &    (0.0139)         &    (0.0163)         &    (0.0144)         \\
\hline
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         \\
Observations        &12,137,175         &3,284,329         &8,852,845         \\
Mean of DV          &      0.1707         &      0.1188         &      0.1899         \\
$R^2$               &      0.0020         &      0.0014         &      0.0025         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table provides a robustness test for our main findings by substituting borrowers' race with ZCTA5 demographic data, as opposed to our method of matching with HMDA. The robustness tests follow our main specification (Column (3)) of Table \ref{table:4}. Columns (1-3) show the results for the full sample, mortgagors, and non-mortgagors, respectively (mortgagors are anyone with a mortgage at some point in our data). The coefficients represent the effect (in percentage point units) of changing from a ZCTA5 with zero minority population share to one with 100\% minority residents. The data comprises credit bureau records from 2013–2017. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/table_4_b.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and New Petitioned Judgments}\label{table:4b}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{6}{c}{Petitioned Judgment}\\

\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female               &      0.0078         &      0.0014         &      0.0036         &      0.0050         &      0.0185         &     -0.0019         \\
                    &    (0.0082)         &    (0.0098)         &    (0.0098)         &    (0.0104)         &    (0.0399)         &    (0.0049)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority             &      0.0464\sym{***}&      0.0555\sym{***}&      0.0220         &      0.0192         &      0.0575         &      0.0031         \\
                    &    (0.0132)         &    (0.0180)         &    (0.0178)         &    (0.0186)         &    (0.0572)         &    (0.0077)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age               &     -0.0009\sym{***}&     -0.0015\sym{***}&     -0.0002         &     -0.0005         &     -0.0009         &      0.0001         \\
                    &    (0.0002)         &    (0.0003)         &    (0.0003)         &    (0.0003)         &    (0.0014)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$  &                     &                     &     -0.0013\sym{***}&     -0.0014\sym{***}&     -0.0025\sym{***}&     -0.0002\sym{***}\\
                    &                     &                     &    (0.0001)         &    (0.0001)         &    (0.0004)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$          &                     &                     &      0.0011\sym{**} &      0.0013\sym{**} &      0.0008         &      0.0001         \\
                    &                     &                     &    (0.0004)         &    (0.0005)         &    (0.0006)         &    (0.0002)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$          &                     &                     &     -0.0001\sym{***}&     -0.0002\sym{***}&     -0.0004\sym{***}&     -0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0000)         &    (0.0001)         &    (0.0000)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Outstanding Judgment$_{t-1}$  &                     &                     &     -0.0466         &     -0.0639         &     -0.4568\sym{***}&      0.0137         \\
                    &                     &                     &    (0.0639)         &    (0.0658)         &    (0.0904)         &    (0.1340)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.1005\sym{***}&      0.1293\sym{***}&      0.9873\sym{***}&      1.0548\sym{***}&      1.8057\sym{***}&      0.1843\sym{***}\\
                    &    (0.0125)         &    (0.0160)         &    (0.0794)         &    (0.0862)         &    (0.2271)         &    (0.0428)         \\
\hline
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)           &      0.0615         &      0.0615         &      0.0615         &      0.0615         &      0.2370         &      0.0087         \\
$R^2$               &      0.0001         &      0.0343         &      0.0356         &      0.0366         &      0.0707         &      0.0277         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment petitioned. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, while Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 6 and 7 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/table_4_c.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and New Satisfied Judgments}\label{table:4c}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{6}{c}{Satisfied Judgment}\\

\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female          &            0.0080         &      0.0046         &      0.0063         &      0.0065         &     -0.0140         &      0.0090\sym{*}  \\
                    &    (0.0053)         &    (0.0060)         &    (0.0061)         &    (0.0064)         &    (0.0213)         &    (0.0050)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority      &      0.0222\sym{**} &      0.0282\sym{***}&      0.0120         &      0.0068         &      0.0152         &      0.0062         \\
                    &    (0.0091)         &    (0.0106)         &    (0.0103)         &    (0.0106)         &    (0.0253)         &    (0.0090)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age              &     -0.0006\sym{***}&     -0.0005\sym{**} &     -0.0003         &     -0.0003         &     -0.0012         &      0.0000         \\
                    &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0007)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$ &                     &                     &     -0.0002\sym{***}&     -0.0002\sym{***}&     -0.0003\sym{**} &     -0.0001\sym{**} \\
                    &                     &                     &    (0.0000)         &    (0.0001)         &    (0.0002)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$  &                     &                     &     -0.0002         &     -0.0004\sym{**} &     -0.0003         &     -0.0001         \\
                    &                     &                     &    (0.0002)         &    (0.0001)         &    (0.0002)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$      &                     &                     &     -0.0000         &     -0.0000         &     -0.0001         &      0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0000)         &    (0.0001)         &    (0.0000)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Outstanding Judgment$_{t-1}$    &                     &                     &      0.6217\sym{***}&      0.6125\sym{***}&      0.5891\sym{***}&      1.1462\sym{***}\\
                    &                     &                     &    (0.0775)         &    (0.0786)         &    (0.0920)         &    (0.2722)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.0494\sym{***}&      0.0449\sym{***}&      0.1673\sym{***}&      0.1784\sym{***}&      0.2965\sym{***}&      0.0897\sym{**} \\
                    &    (0.0086)         &    (0.0089)         &    (0.0353)         &    (0.0384)         &    (0.1065)         &    (0.0383)         \\
\hline
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)         &      0.0249         &      0.0249         &      0.0249         &      0.0249         &      0.0830         &      0.0073         \\
$R^2$               &      0.0001         &      0.0334         &      0.0379         &      0.0392         &      0.0762         &      0.0373         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment satisfied. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, while Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 6 and 7 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

